Learning From Long-Tailed Data With Noisy Labels

Class imbalance and noisy labels are the norm rather than the exception in many large-scale classification datasets. Nevertheless, most works in machine learning typically assume balanced and clean data. There have been some recent attempts to tackle, on one side, the problem of learning from noisy labels and, on the other side, learning from long-tailed data. Each group of methods make simplifying assumptions about the other. Due to this separation, the proposed solutions often underperform when both assumptions are violated. In this work, we present a simple two-stage approach based on recent advances in self-supervised learning to treat both challenges simultaneously. It consists of, first, task-agnostic self-supervised pre-training, followed by task-specific fine-tuning using an appropriate loss. Most significantly, we find that self-supervised learning approaches are effectively able to cope with severe class imbalance. In addition, the resulting learned representations are also remarkably robust to label noise, when fine-tuned with an imbalance- and noise-resistant loss function. We validate our claims with experiments on CIFAR-10 and CIFAR-100 augmented with synthetic imbalance and noise, as well as the large-scale inherently noisy Clothing-1M dataset.

==> 04-ELR.tex <==
\subsection*{Understanding Memorization and Learning in Long-Tailed Data with Noisy Labels}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figs/CE_bal.png}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figs/CE_imb.png}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figs/ELR_bal.png}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figs/ELR_imb.png}
\end{figure}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/ELR_1.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/ELR_2.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/ELR_3.png}
     \end{subfigure}
    \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/ELR_4.png}
     \end{subfigure}
    \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/ELR_5.png}
     \end{subfigure}

\end{figure}

==> 04-table1.tex <==
%\begin{table}[t]
%\centering
%\begin{tabular}{l|lllll|lllll}
%\toprule
\begin{table}[]
\begin{center}
\begin{tabular}{l|llll|llll} \toprule
              & \multicolumn{4}{|c}{CIFAR-10} & \multicolumn{4}{|c}{CIFAR-100} \\ \cline{2-9}
Method        & 20\% & 50\% & 80\% & 90\% & 20\% & 50\% & 80\% & 90\% \\ \hline %\midrule
Cross-Entropy & 82.7 & 57.9 & 26.1 & 16.8  & 61.8 & 37.3 & 8.8  & 3.5\\
Meta Learning~\cite{rusu19metalearning} 
              & 92.0 & 88.8 & 76.1 & 58.3  & 67.7 & 58.0 & 40.1 & 14.3 \\
DivideMix~\cite{li2020dividemix} 
              & 95.7 & 94.4 & 92.9 & 75.4  & 76.9 &{\bf 74.2} & 59.6 & 31.0\\
ELR~\cite{liu2020early} 
              & {\bf 95.8} &{\bf 94.8}&{\bf 93.3}& 78.7  & {\bf 77.6} & 73.6 & {\bf 60.8} & 33.4\\ \hline
SimCLR (ours) & 89.2 & 88.7 & 88.0 & 86.0  & 61.0 & 59.5 & 53.9 & 47.7\\
Barlow Twins (ours) & 90.1 & 88.1 & 86.5 & 79.0 & 65.8 & 58.8 & 55.5 & 50.1\\
BYOL (ours)   & 92.0  & 90.5 & 85.1 & 65.7 & 68.7 & 63.2 & 55.1 & 40.9 \\
SimSiam (ours)& 91.4 & 90.2 & 88.9 &{\bf 88.1} & 66.0 & 63.8 & 57.1 & {\bf 53.0} \\
\bottomrule
\end{tabular}
\label{tab:cifar_balanced}
\vspace{0.5em}
\caption{CIFAR-10 and CIFAR-100 Results for symmetric noise on balanced data.}
\label{tab:balanced}
\end{center}
\end{table}


==> 04-table2.tex <==
\begin{table*}[]
\begin{center}
\begin{tabular}{@{}l|lllll|lllll@{}}
\toprule
              & \multicolumn{5}{|c}{$\gamma=50$} & \multicolumn{5}{|c}{$\gamma=100$} \\ \cline{2-11}
Method        & 20\% & 40\% & 60\% & 80\% & 90\% & 20\% & 40\% & 60\% & 80\% & 90\% \\ \midrule
DivideMix~\cite{li2020dividemix}
              & 73.8 & 66.2 & 59.1 & 55.3 & 29.2 & 59.7 & 56.7 & 50.7 & 41.6 & 21.2 \\
ELR~\cite{liu2020early}
              & 63.1 & 53.7 & 33.7 & 25.1 & 23.5 & 51.6 & 36.0 & 27.0 & 24.6 & 23.5 \\
 \midrule
SimCLR (ours)  & 74.8 & 71.7 &{\bf 68.4}&{\bf 61.4}&{\bf 55.3}& 70.4 & 66.6 & 61.0 & 54.7 & 42.9\\
Barlow Twins (ours) & 73.2 & 70.1 & 64.5 & 52.2 & 35.2 & 68.7 & 65.4 & 59.7 & 47.0 & 32.9 \\
BYOL (ours)   &{\bf 77.3}&{\bf 74.1}& 65.1 & 49.2 &	35.1 &{\bf 72.1}&{\bf 68.1}& 61.4 &	43.8 & 29.7 \\ 
SimSiam (ours) & 74.5 & 72.3 & 65.9 & 56.5 & 54.3 & 71.5 &{\bf 68.1}&{\bf 61.5}&{\bf 54.8}&{\bf 48.8}\\ 

\bottomrule
\end{tabular}
\vspace{1em}
\caption{Results on long-tailed version of CIFAR-10, $\gamma=50$ and $\gamma=100$}
\label{tab:cifar_long}
\end{center}
\end{table*}



==> 04-table3.tex <==
\begin{table}[h]
\centering
\begin{tabular}{l|lllll|lllll}
\toprule
              & \multicolumn{5}{|c}{$\gamma=5$} & \multicolumn{5}{|c}{$\gamma=10$} \\ \cline{2-11}
Method        & 20\% & 40\% & 60\% & 80\% & 90\% & 20\% & 40\% & 60\% & 80\% & 90\% \\ \midrule
DivideMix~\cite{li2020dividemix}
              &{\bf 68.5}&{\bf 64.1}&{\bf 55.6}& 31.4 & 12.2 &{\bf 62.6}&{\bf 58.1}&{\bf 47.4}& 26.1 & 10.0\\
ELR~\cite{liu2020early}
              & 56.8 & 46.2 & 30.1 & 11.2 & 5.5  & 48.4 & 34.7 & 22.6 & 9.2  & 4.7\\
\midrule             
SimCLR (ours) & 54.3 & 51.9 & 48.6 & 42.3 & 35.4 & 50.4 & 47.8 & 44.4 &{\bf 37.6}&{\bf 29.4}\\
Barlow Twins (ours) & 55.3 & 52.3 & 49.4 & 42.6 & 32.6 & 50.7 & 47.2 & 43.3 & 35.0 & 23.4 \\
BYOL (ours)   & 58.6 & 55.5 & 48.2 & 36.3 &	21.8 & 54.8 & 50.6 & 42.8 &	28.4 & 15.9 \\ 
SimSiam (ours) & 56.2 & 53.8 & 48.6 &{\bf 42.3}&{\bf 37.2}& 51.1 & 48.2 & 42.6 & 35.8 & 27.9\\ 


\bottomrule
\end{tabular}
\vspace{0.5em}
\caption{Results on Long-Tailed version of CIFAR-100, $\gamma=5$, $\gamma=10$.}
\label{tab:cifar100_long}

\end{table}



==> old-table_cifar10.tex <==
% \begin{table}[]
% \begin{tabular}{@{}lllllll@{}}
% \toprule
% Method/Noise           & 0\%   & 20\%  & 40\%  & 60\%  & 80\%  & 90\%  \\ \midrule
% SimCLR+Logit+SuperLoss & 79.01 & 76.78 & 72.32 & 64.95 & 53.08 & 41.38 \\
% -Logit                 & 71.52 & 67.57 & 63.65 & 58.34 & 51.15 & 41.26 \\
% -SuperLoss             & 79.67 & 75.48 & 71.52 & 63.46 & 46.96 & 30.32 \\ \bottomrule
% \end{tabular}
% \vspace{1em}
% \caption{Ablation Study on CIFAR-10 with $\gamma=50$}
% \label{tab:cifar10_ablation}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table}[]
% \begin{tabular}{@{}lllllll@{}}
% \toprule
% Method/Noise            & 0\%   & 20\%  & 40\%  & 60\%  & 80\%  & 90\%  \\ \midrule
% ELR                     & 75.64 & 62.69 & 52.86 & 38.79 & 27.93 & 22    \\
% SimCLR+Logit+SuperLoss  & 77.59 & 74.41 & 72.13 & 69.47 & 62.84 & 55.7 \\ 
% SimSiam+Logit+SuperLoss & 76.45 & 74.51 & 72.33 & 65.93 & 56.53 & 54.30 \\ \bottomrule
% \end{tabular}
% \vspace{1em}
% \caption{Results on CIFAR-10 with $\gamma=50$}
% \label{tab:cifar10_ablation}
% \end{table}

% \begin{table}[]
% \begin{tabular}{@{}lllll@{}}
% \toprule
% Method/Noise            & 20\%  & 40\%  & 60\%  & 80\%  \\ \midrule
% ELR                     & 48.42 & 34.69 & 22.67 & 9.21  \\
% DivideMix               & 62.62 & 58.15 & 47.42 & 26.06 \\
% SimCLR+Logit+SuperLoss  & 50.80 & 48.16 & 45.05 & \textbf{37.67} \\ 
% SimSiam+Logit+SuperLoss & 51.09 & 48.23 & 42.61 & 35.81 \\ \bottomrule
% \end{tabular}
% \vspace{1em}
% \caption{Results on CIFAR-100 with $\gamma=10$}
% \label{tab:cifar100_10}
% \end{table}


==> old_table_cifar100.tex <==
% \begin{table}[]
% \centering
% \begin{tabular}{@{}lllll@{}}
% \toprule
% Method/Noise Ratio & 20\% & 50\% & 80\% & 90\% \\ \midrule
% Cross-Entropy      & 61.8 & 37.3 & 8.8  & 3.5  \\
% Meta Learning~\cite{rusu19metalearning}      & 67.7 & 58.0 & 40.1 & 14.3 \\
% DivideMix~\cite{li2020dividemix}          & 76.9 & 74.2 & 59.6 & 31.0 \\
% ELR+~\cite{liu2020early}               & 77.6 & 73.6 & 60.8 & 33.4 \\
% SimCLR             & 61.0 & 59.5 & 53.8 & 85.9 \\
% SimSiam            & 66.0 & 63.8 & 57.1 & 53.0 \\ \bottomrule
% \end{tabular}
% \vspace{1em}
% \caption{Results for Symmetric Noise on CIFAR-100}
% \end{table}
% \begin{table}[]
% \begin{tabular}{@{}lllllllll@{}}
% \toprule
% Method/Noise-Ratio & \multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}20\%\\ Best    Last\end{tabular}} & \multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}50\%\\ Best    Last\end{tabular}} & \multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}80\%\\ Best    Last\end{tabular}} & \multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}90\%\\ Best    Last\end{tabular}} \\ \midrule
% Cross-Entopy & 86.8 & 82.7 & 79.4 & 57.9 & 62.9 & 26.1 & 42.7 & 16.8 \\
% Meta-Learning~\cite{rusu19metalearning} & 92.9 & 92.0 & 89.3 & 88.8 & 77.4 & 76.1 & 58.7 & 58.3 \\
% DivideMix~\cite{li2020dividemix} & 96.1 & 95.7  & 94.6 & 94.4 & 93.2  & 92.9 & 76.0 & 75.4\\
% ELR+~\cite{liu2020early} & ---  & 95.8 & --- & 94.8 & ---  & 93.3 & --- & 78.7 \\
% SimCLR+SuperLoss (our) & 89.1  & 89.1 & 88.69 & 88.58 & 87 & 86.33 & 84.15 & 80.61 \\ 
% SimSiam+SuperLoss (our) & --- & 91.44 & --- & 90.21 & --- & 88.89 & --- & \textbf{88.09}\\ \bottomrule
% \end{tabular}
% \vspace{1em}
% \caption{Results for Symmetric Noise on CIFAR-10}
% \label{tab:cifar10_balanced}
% \end{table}

% \begin{table}[]
% \begin{tabular}{@{}lllllllll@{}}
% \toprule
% Method/Noise-Ratio & \multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}20\%\\ Best    Last\end{tabular}} & \multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}50\%\\ Best    Last\end{tabular}} & \multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}80\%\\ Best    Last\end{tabular}} & \multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}90\%\\ Best    Last\end{tabular}} \\ \midrule
% Cross-Entopy       & 62.0                                   & 61.8                                   & 46.7                                   & 37.3                                   & 19.9                                   & 8.8                                    & 10.1                                   & 3.5                                    \\
% Meta-Learning      & 68.5 & 67.7 & 59.2 & 58.0 & 42.4 & 40.1 & 19.5 & 14.3\\
% DivideMix & 77.3  & 76.9 & 74.6 & 74.2 & 60.2 & 59.6 & 31.5 & 31.0\\
% ELR+ & --- & 77.6 & ---  & 73.6 & --- & 60.8 & ---  & 33.4 \\
% SimCLR+Logit+SuperLoss   & 61.01 & 61.01 & 59.73 & 59.54 & 54.39 & 52.92 & 49.2 & 44.29 \\
% SimSiam+Logit+SuperLoss & --- & 66.02 & --- & 63.84 & --- & 57.13 & --- & \textbf{53} \\ \bottomrule
% \end{tabular}
% \vspace{1em}
% \caption{Results for Symmetric Noise on CIFAR-100}
% \label{tab:cifar100_balanced}
% \end{table}

==> target_imbalance.tex <==
\section*{ELR regularization and class bias}

ELR regularization (Eq. 6, ELR paper) does a great job in class balance. However, under class imbalance 
it works for dominant classes only. We have already tried to replace the Cross Entropy loss with Focal and Logit Adjusted losses.

Below there is a couple of proposals to tune the regularization term under class imbalance.

\paragraph{Biased target estimation}
The first proposal is inspired by~\cite{hyun2020class}; they analyzed the impact of the severe class imbalance on the Mean Teacher in semi-supervised learning and argued that "performance degradation is evident in the minor class", "conventional consistency regularization-based
methods are generally expected to degrade the performance for the minor class". They proposed to suppress consistency loss and to make the model more conservative for small classes.

\cite{hyun2020class} worked with model parameters $\theta$ directly. Making a bridge to the target estimation in Eq.9 in ELR paper, the idea is to tune the momentum $\beta$ in the function of the predicted class:

\begin{equation}
{\bf t}^i (k) := \beta^z {\bf t}^i(k-1) + (1- \beta^z) {\bf p}^i(k)
\label{eq:temp_biaz}
\end{equation}
where $z= \frac{1+\alpha_c}{2}$, $\alpha_c=\frac{n_c}{n_{max}}$, $c=\argmax( {\bf p}^i(k))$, $n_c$ is the number of examples of the class predicted by the model, $n_{max}$ is the number of samples of the dominant class ( with the most frequency). 

For the dominant class, $\alpha_c \approx 1$ and Eq. \ref{eq:temp_biaz} is identical to Eq.9 in ELR. For a small class, $\alpha_c \approx 0$, $z \approx 0.5$ and the weight of new prediction in the temporal assembling becomes smaller, $1-\beta^{0.5}$ instead of $1-\beta$.

{\bf Disclaimer.} Note that~\cite{hyun2020class} does not assume any class noise, like us, and estimation of the class samples might be quite misleading.
